Effective Black Box Testing of Sentiment Analysis Classification Networks

Transformer-based neural networks have demonstrated remarkable performance in natural language processing tasks such as sentiment analysis. Nevertheless, the issue of ensuring the dependability of these complicated architectures through comprehensive testing is still open. This paper presents a collection of coverage criteria specifically designed to assess test suites created for transformer-based sentiment analysis networks. Our approach utilizes input space partitioning, a black-box method, by considering emotionally relevant linguistic features such as verbs, adjectives, adverbs, and nouns. In order to effectively produce test cases that encompass a wide range of emotional elements, we utilize the k-projection coverage metric. This metric minimizes the complexity of the problem by examining subsets of k features at the same time, hence reducing dimensionality. Large language models are employed to generate sentences that display specific combinations of emotional features. The findings from experiments obtained from a sentiment analysis dataset illustrate that our criteria and generated tests have led to an average increase of 16\% in test coverage. In addition, there is a corresponding average decrease of 6.5\% in model accuracy, showing the ability to identify vulnerabilities. Our work provides a foundation for improving the dependability of transformer-based sentiment analysis systems through comprehensive test evaluation.

==> background.tex <==

% todo(pouria): maybe it is better to name this section "related works".
% Background is used for definitions that we need to learn to understand the methodology.
\section{Background}\label{ssec:Background}
This section is divided into two parts: firstly, it provides a definition of sentiment analysis and explains its role in neural networks; secondly, it discusses the methods of testing employed to accomplish this task and the chosen strategy. Our goal is to improve our understanding of the essential information and abilities required to effectively comprehend sentiment analysis and implement comprehensive testing of it.
\subsection{Sentiment analysis}\label{sssec:Sentiment analysis}

Sentiment analysis is a natural language processing (NLP) activity that seeks to identify the emotional sentiment conveyed in a given text. Emotional sentiment analysis is a distinct branch of sentiment analysis that concentrates on examining the precise emotions conveyed in a given text. Tweets are commonly favored as the main source for sentiment analysis projects because of their succinct and expressive characteristics, which make them well-suited for collecting a wide range of emotional responses. The neural network is designed with a specific purpose of identifying and categorizing various emotions, such as grief, joy, surprise, and others, that are present in the provided text. The progress in neural networks, including the augmentation of model complexity and the utilization of larger training datasets, has resulted in a significant improvement in the precision and efficacy of sentiment analysis tasks. Neural networks, particularly those utilizing transformer architectures such as Distil-bert, Roberta, and XLnet, go through training for this specific purpose with remarkable precision. For example, a comprehensive test suite may include diverse datasets, edge cases, and stress tests to thoroughly evaluate the neural networks' performance. To evaluate the effectiveness of these networks, it is essential to utilize traditional software engineering testing approaches.

\subsection{ Testing}\label{sssec: Testing}

There are ways to check if test suites are complete, such as neuron coverage for convolutional neural networks (CNNs), which counts how many neurons are activated by each input and checks if test suites are complete by counting how many neurons are activated in the internal structure by each test. \cite{Neuron} In the context of RNNs, the coverage metric entails considering inputs as the fundamental unit of test coverage, analogous to how neuron coverage is viewed in CNNs. Various studies have suggested certain coverage criteria, such as Hidden State Coverage (HS-C), Boundary Coverage (BC), Stepwise Coverage (SC), and Temporal Coverage (TC), to provide direction for testing Recurrent Neural Networks (RNNs).\cite{RNNCOVER} Nevertheless, the testing methods for RNNs are currently more restricted in comparison to CNNs, and the architecture of RNNs necessitates specialized coverage measures that are customized for their network topology. [1] [2]. However, the implementation of these measures is not feasible for transformers due to their complicated nature and the presence of millions of trainable characteristics. To assess the completeness of test suites for these networks, we need to utilize coverage metrics from software engineering. These metrics analyze test suites without considering the internal architecture of the system-under-test (SOT), which in the current instance entails transformers. We can employ metrics that consider the system as a black-box, which is formally referred to as black-box testing. This approach involves utilizing techniques like input space partitioning to find specific portions of the system that necessitate additional testing. It achieves this by designing input spaces and thoroughly examining them. This approach has been utilized for sentiment analysis in this paper, and it will be comprehensively detailed in Section 3.

==> discussion.tex <==
\section{Discussion}

==> feature-work.tex <==
\section{Feature Works}\label{ssec:future work}
There are several promising directions for extending this research. First, exploring the applicability of our coverage criteria to other transformer-based natural language processing tasks, such as text summarization or machine translation, could provide valuable insights into their effectiveness.

Expanding the scope of linguistic elements beyond verbs, adjectives, adverbs, and nouns could enhance the criteria's ability to detect subtle emotional nuances, including negations and emojis used in text.

Furthermore, incorporating advanced techniques like metamorphic testing or mutation testing could complement our approach, offering additional methods to systematically assess the robustness and reliability of sentiment analysis models.

Lastly, investigating the scalability and computational efficiency of our methodology on larger datasets and more complex transformer architectures would be crucial for extending its practical applicability to real-world, industry-scale scenarios.



==> intro.tex <==
\section{Introduction}\label{sec:introduction}

The impact of neural networks on various fields, including image recognition, natural language processing, and self-driving cars, has been significant~\cite{wu}. In the context of Natural Language Processing (NLP), neural networks have gained notable recognition due to their ability to enhance accuracy~\cite{Chen_2020}.
Sentiment analysis, also known as opinion mining or emotion AI, is a natural language processing (NLP) technique used to determine the emotional tone or subjective opinion expressed in text.  This procedure utilizes NLP methodologies to analyze and interpret human language, enabling diverse applications across various domains. For instance, in marketing, sentiment analysis can be leveraged to evaluate customer opinions about products and services, providing valuable insights for brand reputation management. 
Several tools, such as Stanford CoreNLP~\cite{manning2014stanford}, NLTK~\cite{bird2006nltk}, and TextBlob~\cite{loria2018textblob}, are utilized to comprehend customer sentiment and harness the emotions embedded within it. This strategy is also commonly applied in the evaluation of mental health, as highlighted in Adil Rajput's 2020 study~\cite{rajput2020natural}.

Traditional emotion recognition methods often struggle with the inherent complexities of human language~\cite{kong2024research}. These complexities include word ambiguity, where a word's emotional connotation can shift depending on context (e.g., ``scared'' can be positive in an exciting situation or negative in a threatening one). In addition, sarcasm and negation pose challenges in identifying true sentiment.  Furthermore, the process of understanding emotional meaning must include evaluating words that are not directly close to each other in a sentence, which is a step away from traditional methods.

Transformer-based neural networks effectively handle the ambiguity in emotion sentiment analysis through their attention mechanisms and large parameters~\cite{vaswani2017attention}. Parallel text processing allows them to analyze text data efficiently and capture the hidden emotional factors that can exist across longer distances within a sentence. Through pre-training on extensive datasets, transformers are capable of learning complex language patterns and the subtle details of human emotional expression~\cite{vaswani2017attention}.

To guarantee the efficacy of these complex models, comprehensive testing protocols are essential. A significant challenge lies in evaluating the sufficiency of test suites specifically designed for Transformer-based emotional sentiment analysis networks. Given their complex architecture and the large number of parameters, conventional methods like neuron coverage~\cite{deepgauge} seem to be impractical. To address this limitation, we introduce in this work a novel set of coverage criteria designed to evaluate test suites for the assessment of Transformer-based emotion sentiment analysis networks. We employ the principle of input space partitioning, segmenting textual data into emotionally-relevant categories. This strategy enables us to concentrate on particular areas of the input space and generate targeted test cases.

To achieve high coverage with the least number of test cases, we employ the k-projection coverage method~\cite{k-project}. This technique utilizes dimensionality reduction by examining smaller feature sets at the same time. Concentrating on these smaller subsets allows for an efficient evaluation of the network's performance across diverse emotional categories within the input space. This strategy ensures comprehensive coverage with fewer tests, thereby eliminating the necessity for extensive test suites.
Additionally, we introduce a set of specialized features specifically designed for emotional sentiment analysis. These features capture the emotional details within text data, thereby aiding the network in accurately identifying the intended emotions.


Upon applying our emotion-specific k-projection coverage method to a dataset designed for emotional sentiment analysis, we observed a 14\% average increase in coverage of the generated sentences. This enhanced coverage led to a 5\% decrease in the accuracy of the System-Under-Test (SUT) on the new test suites, demonstrating the effectiveness of our approach in uncovering additional faults.
% The presented methodology has a number of advantages that combine to increase the accuracy of Transformer-based emotion sentiment analysis networks. First, by using the k-projection coverage method, the number of test cases required for comprehensive coverage is reduced. This leads to improved efficiency by allowing the network's performance to be evaluated with a smaller set of tests. Second, input space partitioning allows for targeted testing by focusing on specific emotional aspects of the data. This ensures that the test cases cover the range of emotional categories that the network is likely to encounter in real-life scenarios. 

The contributions of our study are as follows: 
\begin{enumerate}
    \item We introduce novel coverage criteria based on k-projection for black-box testing of sentiment analysis systems. This metric serves a dual purpose: evaluating the effectiveness of existing test suites and guiding the generation of new test cases to augment them.
\item Our experimental results demonstrate that enriching test suites using this proposed coverage criterion leads to a significant reduction in model accuracy. This finding has two key implications:
\begin{itemize}
    \item The coverage criterion is a valid metric for assessing test suites in this context, as higher coverage scores correlate with a greater ability to uncover faults and decrease model accuracy.
\item The coverage criterion can be effectively utilized to generate effective test cases that reveal failures and thus improve the overall quality of test suites.
\end{itemize}

\end{enumerate}

The remainder of this paper is organized as follows. We explain the proposed methodology in Section~\ref{sec:methodology}, followed by a presentation of the experimental results in Section~\ref{ssec:evaluation}. Section~\ref{ssec:Related Work} discusses related work in the field, and Section~\ref{sec:conclusion} concludes the paper by summarizing our findings and future work described in  \ref{ssec:future work}.
